Automatic Description Generation from Images: A Survey of Models, Datasets, and Evaluation Measures

Automatic description generation from natural images is a challenging problem that has recently received a large amount of interest from the computer vision and natural language processing communities. In this survey, we classify the existing approaches based on how they conceptualize this problem, viz., models that cast description as either generation problem or as a retrieval problem over a visual or multimodal representational space. We provide a detailed review of existing models, highlighting their advantages and disadvantages. Moreover, we give an overview of the benchmark image datasets and the evaluation measures that have been developed to assess the quality of machine-generated image descriptions. Finally we extrapolate future directions in the area of automatic image description generation.

==> introduction_old.tex <==
% !TEX root = review.tex
% INTRODUCTION
\section{Introduction}
The fields of computer vision (CV) and natural language processing (NLP) have seen great advances since the early attempts to use computers for analyzing and interpreting visual data and for understanding and processing human language, respectively. Both emerged from the discipline of Artificial Intelligence and thus share common historical roots. However, CV and NLP are generally considered independent disciplines and even disjoint fields. Both vision and language play essential roles in perceiving the external world that we live in, and we meet multimodal data containing both visual and linguistic elements in our daily lives (for example, tagged images, photos with captions, webpages and subtitled videos). However, the vast majority of current approaches in both CV and NLP do not exploit the joint nature of visual and linguistic information.

Generating automatic descriptions from images is a task that can only be performed successfully if both visual and linguistic information are processed. The task has recently attracted the attention from both %BP repetitive computer vision and natural language processing 
communities, leading to a rapidly evolving body of research. In its simplest form, \emph{automatic image description} can be defined as the problem of associating images with natural language text by recognizing and verbalizing the visual content within an image (Figure~\ref{fig:system}). In other words, a model analyzes the images to produce a sentence or sentences describing the salient objects or actions that appear in them. A number of important challenges arise. First and foremost, solving this problem needs a tight coupling of CV and NLP approaches to enable joint processing of visual and linguistic data. Secondly, visual and linguistic data both have inherent ambiguities, which need to be resolved independently or jointly, in order to come up with valid descriptions.

\begin{figure}
\centerline{\includegraphics[width=0.9\columnwidth]{system}} 
\caption{Automatic image description systems.}
\label{fig:system}
\end{figure}

Since the origins of computer vision, which can be traced to Seymour Papert's Summer Vision Project~\cite{Papert1966} at MIT, the grand goal of CV is to design machines which can interpret images  like humans do. % and like humans and reason about the word perceived through their eyes. 
Until a few years ago, most of the research effort in computer vision has focused on %BP see issue 12: introduce rest/following paragraphs here: early days just assigning atomic categories/labels, then extend with attributes (from nominals only to adjectives etc), then further to generation of entire descriptions/sentences
\textcolor{red}{matching words with images}~\cite{Mori1999,Duygulu2002,Datta2008}. To give an example, % BP rewrite the example, superlong sentence
 a large number of researchers have tackled the object detection aspect of visual scene understanding, where the main task is to discover an image region which can be associated with a label referring to an object class from a pre-determined set of visual classes~\cite{Everingham2010,Everingham2015}. Interestingly, most of these object detectors have employed techniques inspired by the NLP literature. For instance, they commonly use bag of word-based visual representations~\cite{Fergus2003,Grauman2005,Lazebnik2006} as features, or employ compositional part models to describe an object in terms of its parts in a hierarchical way~\cite{Felzenszwalb2010}. 

More recent studies have begun to broaden the field by extending the scope of recognition with the estimation of common attributes of the objects or scene regions such as ``tall'', ``man-made'',``dry'', etc.\ \cite{Ferrari2007,Farhadi2009,Lampert2009,Wang2009,Berg2010,Rohrbach2010,Parikh2011,Sadeghi2011}. These characteristics provide mid-level semantic information about the entities that are shared across different visual categories. Providing a list of recognized objects and their attributes in a scene is usually not enough to understand a scene, as there are certain other things that needs to be explored as well, such as the relationship between the objects. Furthermore, some objects can only be recognized in context, and the shape of some object classes is highly variable. In that regard, another line of research, semantic image segmentation or image parsing, aims at segmenting images into coherent regions and jointly labeling them with the words that describe their semantic visual categories~\cite{Shotton2008,Tighe2010}.

In contrast to this, when one asks a human subject to describe an image, he/she can provide a detailed and vibrant linguistic description. These descriptions typically provide a richer and more profound portrayal of the visual content of the image, compared to a list of object or attribute labels. Humans describe images by referring to the actions, the objects depicted in these actions and their properties, and the relations between them in an accurate and natural way. Being able to generate a human-like description can therefore be regarded as an important step to full image understanding. This goes beyond what object classifiers, attribute detectors, scene type labelers, etc.\ can achieve. %This has been recognized in both the CV and the NLP literature, and recently, a number of models have been proposed for generating natural language descriptions from images in an automatic manner. The latter models differ from each other based on the way they approach the problem . 
 Thus, a large body of recent CV and NLP work focused on generating natural language descriptions from images in an automatic manner. The proposed models differ in the way they approach the problem. We here categorize them into three types.

The first group of models aims at associating descriptions with images by first detecting or predicting the image content in terms of actions, scene types, objects, their attributes, and spatial relations between objects, based on a set of visual features. These models then use this content information to drive a natural language generation system that outputs a description~\cite{Kulkarni2011,Li2011,Yang2011,Mitchell2012,Elliott2013,Kuznetsova14,Yatskar2014,chen:mind14,dona:long14,ElliottDeVries2015,fang15,Karpathy2015,kiros2014,lebret15,mao15,Ortiz2015,Vinyals2015,xu15}. 

% adapt the following to the new division
The second group of models cast the problem as a \textcolor{red}{description transfer or retrieval problem}. That is, to create image descriptions, the models search for images in a database that are visually similar in terms of their content, and then use the description associated with these retrieved images to describe the given input images~\cite{Ordonez2011,Gupta2012,Kuznetsova2012,Mason2014,Patterson2014,Devlin2015,Yagcioglu2015}. 

A related set of approaches solve the description task by learning a common semantic space for visual and linguistic data and use this space to perform cross-modal retrieval~\cite{Farhadi2010,Hodosh2013b,Gong2014,Karpathy2014,Socher2014,Verma2014,chen:mind14,dona:long14,Karpathy2015,kiros2014,lebret15,mao15,Vinyals2015,xu15}. The latter technique is our third class of models.

Generating natural language descriptions from videos presents unique
challenges over and above image-based description, as it additionally
requires analyzing the objects and their attributes and actions in the
temporal dimension. Models that aim to solve description generation from videos have been
proposed as well~\cite{Khan2011,Guadarrama2013,Krishnamoorthy2013,Rohrbach2013,Thomason2014}. However, most existing work on description generation has used static images, and this is what we will focus on in this survey.

%Ourgoal is to group automatic image description models into specific categories and to provide a comprehensive overview of the models in each category. Moreover, we aim to examine the available multimodal image datasets which have been used for benchmarking description generation models and review the evaluation measures that have been used to gauge quality of generated descriptions. Our survey focuses on models for generic images, rather than on description generation techniques tailored to specific domains (for instance, the models that work only on sports images).
In this survey article we a) group automatic image description models into specific categories and to provide a comprehensive overview of the models in each category; b) examine the available multimodal image datasets used for benchmarking description generation models; and c) review evaluation measures that have been used to gauge the quality of generated descriptions. Our survey focuses on models for generic images, rather than description generation techniques tailored to specific domains (for instance, the models that work only on sports images).

The remainder of this article is organized as follows: In Section~\ref{sec:models} we classify and describe the existing description generation models from images and discuss their advantages and disadvantages. Section~\ref{sec:datasets_evaluation} presents image description datasets and reviews evaluation measures that are commonly adopted. In Section~\ref{sec:future_direction}, we discuss possible future directions of research, before concluding in Section~\ref{sec:conclusion}.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "review"
%%% End: 

